Performance Analysis of Mobile Cellular-Connected Drones under Practical Antenna Configurations

Providing seamless connectivity to unmanned aerial vehicle user equipments (UAV-UEs) is very challenging due to the encountered line-of-sight interference and reduced gains of down-tilted base station (BS) antennas. For instance, as the altitude of UAV-UEs increases, their cell association and handover procedure become driven by the side-lobes of the BS antennas. In this paper, the performance of cellular-connected UAV-UEs is studied under 3D practical antenna configurations. Two scenarios are studied: scenarios with static, hovering UAV- UEs and scenarios with mobile UAV-UEs. For both scenarios, the UAV-UE coverage probability is characterized as a function of the system parameters. The effects of the number of antenna elements on the UAV-UE coverage probability and handover rate of mobile UAV-UEs are then investigated. Results reveal that the UAV-UE coverage probability under a practical antenna pattern is worse than that under a simple antenna model. Moreover, vertically-mobile UAV-UEs are susceptible to altitude handover due to consecutive crossings of the nulls and peaks of the antenna side-lobes.

==> acronyms.tex <==

\acro{D2D}{device-to-device}
\acro{SIR}{signal-to-interference-ratio}
\acro{SINR}{signal-to-interference-plus-noise-ratio}
\acro{PCP}{Poisson cluster process}
\acro{CoMP}{coordinated multi-point}
\acro{BS}{base station} 
\acro{MD-CoMP}{macrodiversity CoMP transmission}
\acro{MAC}{medium-access-control}
\acro{JT-CoMP}{joint transmission CoMP}
\acro{CoMP-JT}{coordinated multipoint joint transmission}
\acro{SBS}{small base station}
\acro{MDSD}{multiple devices to the single device}
\acro{MDS}{maximum distance seperable}
\acro{SCN}{small cell network}
\acro{PPP}{Poisson point process}
\acro{TCP}{Thomas cluster process}
\acro{CSI}{channel state information}
\acro{PDF}{probability distribution function}
\acro{PMF}{probability mass function}
\acro{RV}{random variable}
\acro{i.i.d.}{independently and identically distributed}
\acro{MBMS}{multimedia broadcasting multicasting service}
\acro{EE}{energy efficiency}
\acro{HCP}{hard-core placement}
\acro{CCDF}{complementary cumulative distribution function}
\acro{CDF}{cumulative distribution function}
\acro{PC}{probabilistic caching}
\acro{RC}{random uniform caching}
\acro{CPF}{caching popular files} 
\acro{PGFL}{probability generating functional}
\acro{KKT}{Karush-Kuhn-Tucker}
\acro{PGF}{point generating function}
\acro{BPP}{binomial point process}
\acro{3GPP}{3rd Generation Partnership Project}
\acro{UAV}{unmanned aerial vehicle}
\acro{FAA}{Federal Aviation Administration}
\acro{UAS}{unmanned aircraft systems}
\acro{AP}{access point}
\acro{GSM}{Global System for Mobile Communications}
\acro{LTE}{long term evolution}
\acro{IoT}{Internet-of-things}
\acro{UE}{user equipment}
\acro{CNPC}{control and non-payload communication}
\acro{FHD}{full high definition}
\acro{NLoS}{non-line-of-sight}
\acro{LoS}{line-of-sight}
\acro{5G}{fifth-generation}
\acro{MGF}{moment generating function}
\acro{3D}{three-dimensional}
\acro{MIMO}{multiple-input multiple-output}
\acro{CB}{conjugate beamforming}
\acro{AU}{aerial user}
\acro{GU}{ground user}
\acro{CLT}{central limit theorem}
\acro{SE}{spectral efficiency}
\acro{MRT}{maximum ratio transmission}
\acro{ZFBF}{zero-forcing beamforming}
\acro{QoS}{quality of service}
\acro{GBS}{ground base station}
\acro{F-RAN}{fog-radio access network}
\acro{RAN}{radio access network}
\acro{RRH}{remote radio head}
\acro{mmWave}{millimeter wave}
\acro{C&C}{command and control}
\acro{ASE}{area spectral efficiency}
\acro{RWP}{random waypoint}
\acro{AUE}{aerial UE}
\acro{GUE}{ground UE}
\acro{SCDP}{successful content delivery probability}
\acro{ULA}{uniform linear array}
\acro{GTA}{ground-to-air}
\acro{UB}{upper bound}
\acro{LB}{lower bound}
\acro{2D}{two dimensional}
\acro{1D}{one dimensional}
\acro{HARP}{highest average received power}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}

==> newcommands.tex <==

\newcommand{\sinr}{\mathrm{SINR}}
\newcommand{\sir}{\mathrm{SIR}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\Eb}{\mathbb{E}}
\newcommand{\Rb}{\mathbb{R}}
\newcommand{\Rs}{\mathbb{R}^2}
\newcommand{\Rp}{\mathbb{R}^+}
\newcommand{\Lc}{\mathcal{L}}

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\black}{\textcolor{black}}
\newcommand{\magenta}{\textcolor{magenta}}

\newcommand{\Eq}[1]{(\ref{eq:#1})}
\newcommand{\App}[1]{Appendix~\ref{app:#1}}
\newcommand{\Fig}[1]{Fig.~\ref{fig:#1}}

\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\R}{\mathbb{R}}
\DeclareMathOperator*{\N}{\mathcal{N}}
\DeclareMathOperator*{\U}{\mathcal{U}}
\DeclareMathOperator*{\CN}{\mathcal{CN}}

